Photoevaporation and High-Eccentricity Migration Created the Sub-Jovian Desert

The mass-period or radius-period distribution of close-in exoplanets shows a paucity of intermediate mass/size (sub-Jovian) planets with periods ~< 3 days. We show that this sub-Jovian desert can be explained by the photoevaporation of highly irradiated sub-Neptunes and the tidal disruption barrier for gas giants undergoing high-eccentricity migration. The distinctive triangular shape of the sub-Jovain desert result from the fact that photoevaporation is more effective closer to the host star, and that in order for a gas giant to tidally circularise closer to the star without tidal disruption it needs to be more massive. Our work indicates that super-Earths/mini-Neptunes and hot-Jupiters had distinctly separate formation channels and arrived at their present locations at different times.

==> journals_mnras.tex <==
\def\aj{\ref@jnl{AJ}}                   % Astronomical Journal
\def\actaa{\ref@jnl{Acta Astron.}}      % Acta Astronomica
\def\araa{\ref@jnl{ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\ref@jnl{ApJ}}                 % Astrophysical Journal
\def\apjl{\ref@jnl{ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\ref@jnl{ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\ref@jnl{Appl.~Opt.}}           % Applied Optics
\def\apss{\ref@jnl{Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\ref@jnl{A\&A}}                % Astronomy and Astrophysics
\def\aapr{\ref@jnl{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\ref@jnl{A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\ref@jnl{AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\ref@jnl{BAAS}}               % Bulletin of the AAS
\def\bac{\ref@jnl{Bull. astr. Inst. Czechosl.}}
                % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{\ref@jnl{Chinese Astron. Astrophys.}}
                % Chinese Astronomy and Astrophysics
\def\cjaa{\ref@jnl{Chinese J. Astron. Astrophys.}}
                % Chinese Journal of Astronomy and Astrophysics
\def\icarus{\ref@jnl{Icarus}}           % Icarus
\def\jcap{\ref@jnl{J. Cosmology Astropart. Phys.}}
                % Journal of Cosmology and Astroparticle Physics
\def\jrasc{\ref@jnl{JRASC}}             % Journal of the RAS of Canada
\def\memras{\ref@jnl{MmRAS}}            % Memoirs of the RAS
\def\mnras{\ref@jnl{MNRAS}}             % Monthly Notices of the RAS
\def\na{\ref@jnl{New A}}                % New Astronomy
\def\nar{\ref@jnl{New A Rev.}}          % New Astronomy Review
\def\pra{\ref@jnl{Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\ref@jnl{Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\ref@jnl{Phys.~Rev.~C}}        % Physical Review C
\def\prd{\ref@jnl{Phys.~Rev.~D}}        % Physical Review D
\def\pre{\ref@jnl{Phys.~Rev.~E}}        % Physical Review E
\def\prl{\ref@jnl{Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasa{\ref@jnl{PASA}}               % Publications of the Astron. Soc. of Australia
\def\pasp{\ref@jnl{PASP}}               % Publications of the ASP
\def\pasj{\ref@jnl{PASJ}}               % Publications of the ASJ
\def\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
                % Revista Mexicana de Astronomia y Astrofisica
\def\qjras{\ref@jnl{QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\ref@jnl{S\&T}}             % Sky and Telescope
\def\solphys{\ref@jnl{Sol.~Phys.}}      % Solar Physics
\def\sovast{\ref@jnl{Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\ref@jnl{Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\ref@jnl{ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\ref@jnl{Nature}}              % Nature
\def\iaucirc{\ref@jnl{IAU~Circ.}}       % IAU Cirulars
\def\aplett{\ref@jnl{Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\def\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\ref@jnl{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\ref@jnl{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\ref@jnl{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\ref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\def\nphysa{\ref@jnl{Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\ref@jnl{Phys.~Rep.}}   % Physics Reports
\def\physscr{\ref@jnl{Phys.~Scr}}   % Physica Scripta
\def\planss{\ref@jnl{Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\ref@jnl{Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

==> jovian-desert (2)/journals_mnras.tex <==
\def\aj{\ref@jnl{AJ}}                   % Astronomical Journal
\def\actaa{\ref@jnl{Acta Astron.}}      % Acta Astronomica
\def\araa{\ref@jnl{ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\ref@jnl{ApJ}}                 % Astrophysical Journal
\def\apjl{\ref@jnl{ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\ref@jnl{ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\ref@jnl{Appl.~Opt.}}           % Applied Optics
\def\apss{\ref@jnl{Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\ref@jnl{A\&A}}                % Astronomy and Astrophysics
\def\aapr{\ref@jnl{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\ref@jnl{A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\ref@jnl{AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\ref@jnl{BAAS}}               % Bulletin of the AAS
\def\bac{\ref@jnl{Bull. astr. Inst. Czechosl.}}
                % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{\ref@jnl{Chinese Astron. Astrophys.}}
                % Chinese Astronomy and Astrophysics
\def\cjaa{\ref@jnl{Chinese J. Astron. Astrophys.}}
                % Chinese Journal of Astronomy and Astrophysics
\def\icarus{\ref@jnl{Icarus}}           % Icarus
\def\jcap{\ref@jnl{J. Cosmology Astropart. Phys.}}
                % Journal of Cosmology and Astroparticle Physics
\def\jrasc{\ref@jnl{JRASC}}             % Journal of the RAS of Canada
\def\memras{\ref@jnl{MmRAS}}            % Memoirs of the RAS
\def\mnras{\ref@jnl{MNRAS}}             % Monthly Notices of the RAS
\def\na{\ref@jnl{New A}}                % New Astronomy
\def\nar{\ref@jnl{New A Rev.}}          % New Astronomy Review
\def\pra{\ref@jnl{Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\ref@jnl{Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\ref@jnl{Phys.~Rev.~C}}        % Physical Review C
\def\prd{\ref@jnl{Phys.~Rev.~D}}        % Physical Review D
\def\pre{\ref@jnl{Phys.~Rev.~E}}        % Physical Review E
\def\prl{\ref@jnl{Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasa{\ref@jnl{PASA}}               % Publications of the Astron. Soc. of Australia
\def\pasp{\ref@jnl{PASP}}               % Publications of the ASP
\def\pasj{\ref@jnl{PASJ}}               % Publications of the ASJ
\def\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
                % Revista Mexicana de Astronomia y Astrofisica
\def\qjras{\ref@jnl{QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\ref@jnl{S\&T}}             % Sky and Telescope
\def\solphys{\ref@jnl{Sol.~Phys.}}      % Solar Physics
\def\sovast{\ref@jnl{Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\ref@jnl{Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\ref@jnl{ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\ref@jnl{Nature}}              % Nature
\def\iaucirc{\ref@jnl{IAU~Circ.}}       % IAU Cirulars
\def\aplett{\ref@jnl{Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\def\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\ref@jnl{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\ref@jnl{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\ref@jnl{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\ref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\def\nphysa{\ref@jnl{Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\ref@jnl{Phys.~Rep.}}   % Physics Reports
\def\physscr{\ref@jnl{Phys.~Scr}}   % Physica Scripta
\def\planss{\ref@jnl{Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\ref@jnl{Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

==> jovian-desert (2)/ref.tex <==
\begin{thebibliography}{999}

\bibitem[\protect\citeauthoryear{Anderson, Storch, \& Lai}{2016}]{Anderson2016} Anderson K.~R., Storch N.~I., Lai D., 2016, MNRAS, 456, 3671 


\bibitem[Baraffe et al.(2004)]{Baraffe2004} Baraffe, I., Selsis, F., Chabrier, G., et al.\ 2004, \aap, 419, L13 

\bibitem[Baraffe et al.(2010)]{Baraffe2010} Baraffe, I., Chabrier, G., \& Barman, T.\ 2010, Reports on Progress in Physics, 73, 016901


\bibitem[Batygin et al.(2016)]{Batygin2016} Batygin, K., Bodenheimer, P.~H., \& Laughlin, G.~P.\ 2016, \apj, 829, 114 

\bibitem[\protect\citeauthoryear{Beaug{\'e} \& Nesvorn{\'y}}{2012}]{Beauge2012} Beaug{\'e} C., Nesvorn{\'y} D., 2012, ApJ, 751, 119 


\bibitem[Beaug{\'e} \& Nesvorn{\'y}(2013)]{Beauge2013} Beaug{\'e}, C., \& Nesvorn{\'y}, D.\ 2013, \apj, 763, 12 
\bibitem[\protect\citeauthoryear{Bitsch, Lambrechts, \& Johansen}{2015}]{Bitsch2015} Bitsch B., Lambrechts M., Johansen A., 2015, A\&A, 582, A112 



\bibitem[Boley et al.(2016)]{Boley2016} Boley, A.~C., Granados Contreras, A.~P., \& Gladman, B.\ 2016, \apjl, 817, L17

\bibitem[Borucki et al.(2011)]{Borucki2011} Borucki, W.~J., Koch, D.~G., Basri, G., et al.\ 2011, \apj, 736, 19
\bibitem[Cabrera et al.(2017)]{Cabrera2017} Cabrera, J., Barros, S.~C.~C., Armstrong, D., et al.\ 2017, \aap, 606 A75 


\bibitem[Chatterjee et al.(2008)]{Chatterjee2008} Chatterjee, S., Ford, E.~B., Matsumura, S., \& Rasio, F.~A.\ 2008, \apj, 686, 580-602 

\bibitem[Chatterjee \& Tan(2014)]{Chatterjee2014} Chatterjee, S., \& Tan, J.~C.\ 2014, \apj, 780, 53 

\bibitem[\protect\citeauthoryear{Chen \& Rogers}{2016}]{Chen2016} Chen H., Rogers L.~A., 2016, ApJ, 831, 180 



\bibitem[Cumming et al.(2008)]{Cumming2008} Cumming, A., Butler, R.~P., Marcy, G.~W., et al.\ 2008, \pasp, 120, 531 

\bibitem[\protect\citeauthoryear{Dawson \& Johnson}{2018}]{Dawson2018} Dawson R.~I., Johnson J.~A., 2018, arXiv, arXiv:1801.06117 


\bibitem[Dong et al.(2017)]{Dong2017} Dong, S., Xie, J.-W., Zhou, J.-L., Zheng, Z., \& Luo, A.\ 2017, arXiv:1706.07807

\bibitem[\protect\citeauthoryear{Enoch, Collier Cameron, \& Horne}{2012}]{Enoch2012} Enoch B., Collier Cameron A., Horne K., 2012, A\&A, 540, A99 

\bibitem[\protect\citeauthoryear{Fabrycky \& Tremaine}{2007}]{Fabrycky2007} Fabrycky D., Tremaine S., 2007, ApJ, 669, 1298

\bibitem[Ford \& Rasio(2006)]{Ford2006} Ford, E.~B., \& Rasio, F.~A.\ 2006, \apjl, 638, L45 

\bibitem[Fortney et al.(2007)]{Fortney2007} Fortney, J.~J., Marley, M.~S., \& Barnes, J.~W.\ 2007, \apj, 659, 1661 


\bibitem[Fulton et al.(2017)]{Fulton2017} Fulton, B.~J., Petigura, E.~A., Howard, A.~W., et al.\ 2017, \aj, 154, 109 

\bibitem[Fressin et al.(2013)]{Fressin2013} Fressin, F., Torres, G., Charbonneau, D., et al.\ 2013, \apj, 766, 81


\bibitem[Guillochon et al.(2011)]{Guillochon2011} Guillochon, J., Ramirez-Ruiz, E., \& Lin, D.\ 2011, \apj, 732, 74 

\bibitem[Hansen \& Murray(2012)]{Hansen2012} Hansen, B.~M.~S., \& Murray, N.\ 2012, \apj, 751, 158 
\bibitem[H{\'e}brard et al.(2013)]{Hebrard2013} H{\'e}brard, G., Collier Cameron, A., Brown, D.~J.~A., et al.\ 2013, \aap, 549, A134 


\bibitem[Howard et al.(2010)]{Howard2010} Howard, A.~W., Marcy, G.~W., Johnson, J.~A., et al.\ 2010, Science, 330, 653 

\bibitem[\protect\citeauthoryear{Ida \& Lin}{2008}]{Ida2008} Ida S., Lin D.~N.~C., 2008, ApJ, 685, 584-595 

\bibitem[Ionov et al.(2018)]{Ionov2018} Ionov, D.~E., Pavlyuchenkov, Y.~N., \& Shematovich, V.~I.\ 2018, \mnras, 476, 5639 

\bibitem[Jackson et al.(2008)]{Jackson2008} Jackson, B., Greenberg, R., \& Barnes, R.\ 2008, \apj, 678, 1396-1406 

\bibitem[Jackson et al.(2012)]{Jackson2012} Jackson, A.~P., Davis, T.~A., \& Wheatley, P.~J.\ 2012, \mnras, 422, 2024 

\bibitem[Kurokawa \& Kaltenegger(2013)]{Kurokawa2013} Kurokawa, H., \& Kaltenegger, L.\ 2013, \mnras, 433, 3239 

\bibitem[Kurokawa \& Nakamoto(2014)]{Kurokawa2014} Kurokawa, H., \& Nakamoto, T.\ 2014, \apj, 783, 54 

\bibitem[Lammer et al.(2003)]{Lammer2003} Lammer, H., Selsis, F., Ribas, I., et al.\ 2003, \apjl, 598, L121

\bibitem[Laughlin et al.(2011)]{Laughlin2011} Laughlin, G., Crismani, M., \& Adams, F.~C.\ 2011, \apjl, 729, L7

\bibitem[Lee et al.(2014)]{Lee2014} Lee, E.~J., Chiang, E., \& Ormel, C.~W.\ 2014, \apj, 797, 95 



\bibitem[Lee \& Chiang(2016)]{Lee2016} Lee, E.~J., \& Chiang, E.\ 2016, \apj, 817, 90 


\bibitem[Lithwick \& Wu(2014)]{Lithwick2014} Lithwick, Y., \& Wu, Y.\ 2014, Proceedings of the National Academy of Science, 111, 12610 

\bibitem[\protect\citeauthoryear{Lopez \& Fortney}{2013}]{Lopez2013} Lopez E.~D., Fortney J.~J., 2013, ApJ, 776, 2 


\bibitem[Louden et al.(2017)]{Louden2017} Louden, T., Wheatley, P.~J., Irwin, P.~G.~J., Kirk, J., \& Skillen, I.\ 2017, \mnras, 470, 742
\bibitem[Lundkvist et al.(2016)]{Lundkvist2016} Lundkvist, M.~S., Kjeldsen, H., Albrecht, S., et al.\ 2016, Nature Communications, 7, 11201 

\bibitem[Matsakos \& K{\"o}nigl(2016)]{Matsakos2016} Matsakos, T., \& K{\"o}nigl, A.\ 2016, \apjl, 820, L8 


\bibitem[Mazeh et al.(2016)]{Mazeh2016} Mazeh, T., Holczer, T., \& Faigler, S.\ 2016, \aap, 589, A75 

\bibitem[\protect\citeauthoryear{Mu{\~n}oz, Lai, \& Liu}{2016}]{Munoz2016} Mu{\~n}oz D.~J., Lai D., Liu B., 2016, MNRAS, 460, 1086 



\bibitem[\protect\citeauthoryear{Mohanty et al.}{2017}]{Mohanty2018} Mohanty S., Jankovic M.~R., Tan J.~C., Owen J.~E., 2017, arXiv, arXiv:1712.07049 
\bibitem[\protect\citeauthoryear{Mordasini, Alibert, \& Benz}{2009}]{Mordasini2009} Mordasini C., Alibert Y., Benz W., 2009, A\&A, 501, 1139 



\bibitem[Morton et al.(2016)]{Morton2016} Morton, T.~D., Bryson, S.~T., Coughlin, J.~L., et al.\ 2016, \apj, 822, 86


\bibitem[Mulders et al.(2016)]{Mulders2016} Mulders, G.~D., Pascucci, I., Apai, D., Frasca, A., \& Molenda-{\.Z}akowicz, J.\ 2016, \aj, 152, 187 



\bibitem[Murray-Clay et al.(2009)]{MurrayClay2009} Murray-Clay, R.~A., Chiang, E.~I., \& Murray, N.\ 2009, \apj, 693, 23 


\bibitem[\protect\citeauthoryear{Nagasawa, Ida, \& Bessho}{2008}]{Nagasawa2008} Nagasawa M., Ida S., Bessho T., 2008, ApJ, 678, 498-508 
\bibitem[\protect\citeauthoryear{Naoz, Farr, \& Rasio}{2012}]{Naoz2012} Naoz S., Farr W.~M., Rasio F.~A., 2012, ApJ, 754, L36 

\bibitem[Owen \& Jackson(2012)]{Owen2012} Owen, J.~E., \& Jackson, A.~P.\ 2012, \mnras, 425, 2931 

\bibitem[Owen \& Wu(2013)]{Owen2013} Owen, J.~E., \& Wu, Y.\ 2013, \apj, 775, 105 
\bibitem[Owen \& Alvarez(2016)]{Owen2016} Owen, J.~E., \& Alvarez, M.~A.\ 2016, \apj, 816, 34 
\bibitem[Owen \& Menou(2016)]{OMenou16} Owen, J.~E., \& Menou, K.\ 2016, \apjl, 819, L14 

\bibitem[Owen \& Morton(2016)]{OMorton16} Owen, J.~E., \& Morton, T.~D.\ 2016, \apjl, 819, L10 


\bibitem[Owen \& Wu(2017)]{Owen2017} Owen, J.~E., \& Wu, Y.\ 2017, \apj, 847, 29 

\bibitem[Owen \& Murray-Clay(2018)]{OMC18} Owen, J.~E. \& Murray-Clay, R.\ 2018 \mnras,  {\it submitted}

\bibitem[Paxton et al.(2011)]{mesaI} Paxton, B., Bildsten, L., Dotter, A., et al.\ 2011, \apjs, 192, 3 

\bibitem[Paxton et al.(2013)]{mesaII} Paxton, B., Cantiello, M., Arras, P., et al.\ 2013, \apjs, 208, 4 

\bibitem[Paxton et al.(2015)]{mesaIII} Paxton, B., Marchant, P., Schwab, J., et al.\ 2015, \apjs, 220, 15 

\bibitem[Perez-Becker \& Chiang(2013)]{PerezBecker2013} Perez-Becker, D., \& Chiang, E.\ 2013, \mnras, 433, 2294 

\bibitem[Petigura et al.(2013)]{Petigura2013} Petigura, E.~A., Marcy, G.~W., \& Howard, A.~W.\ 2013, \apj, 770, 69 
\bibitem[\protect\citeauthoryear{Petigura et al.}{2018}]{Petigura2018} Petigura E.~A., et al., 2018, AJ, 155, 89 

\bibitem[\protect\citeauthoryear{Petrovich}{2015}]{Petrovich2015} Petrovich C., 2015, ApJ, 805, 75 

\bibitem[Pu \& Valencia(2017)]{Pu2017} Pu, B., \& Valencia, D.\ 2017, \apj, 846, 47 


\bibitem[Rappaport et al.(2012)]{Rappaport2012} Rappaport, S., Levine, A., Chiang, E., et al.\ 2012, \apj, 752, 1 

\bibitem[Ribas et al.(2005)]{Ribas2005} Ribas, I., Guinan, E.~F., G{\"u}del, M., \& Audard, M.\ 2005, \apj, 622, 680 

\bibitem[Sanchis-Ojeda et al.(2015)]{SanchisOjeda2015} Sanchis-Ojeda, R., Rappaport, S., Pall{\`e}, E., et al.\ 2015, \apj, 812, 112 

\bibitem[\protect\citeauthoryear{Sestovic et al.}{2018}]{Sestovic2018} Sestovic, M., Demory, B.~O., Queloz, D., 2018, arXiv, arXiv:1804.03075 


\bibitem[Silburt et al.(2015)]{Silburt2015} Silburt, A., Gaidos, E., \& Wu, Y.\ 2015, \apj, 799, 180 

\bibitem[Syer \& Clarke(1995)]{Syer1995} Syer, D., \& Clarke, C.~J.\ 1995, \mnras, 277, 758 


\bibitem[Szab{\'o} \& Kiss(2011)]{Szabo2011} Szab{\'o}, G.~M., \& Kiss, L.~L.\ 2011, \apjl, 727, L44

\bibitem[Thorngren \& Fortney(2018)]{Thorngren2017} Thorngren, D.~P., \& Fortney, J.~J.\ 2018, \aj, 155, 214 



\bibitem[Tripathi et al.(2015)]{Tripathi2015} Tripathi, A., Kratter, K.~M., Murray-Clay, R.~A., \& Krumholz, M.~R.\ 2015, \apj, 808, 173 

\bibitem[Tu et al.(2015)]{Tu2015} Tu, L., Johnstone, C.~P., G{\"u}del, M., \& Lammer, H.\ 2015, \aap, 577, L3

\bibitem[\protect\citeauthoryear{Valsecchi, Rasio, \& Steffen}{2014}]{Valsecchi2014} Valsecchi F., Rasio F.~A., Steffen J.~H., 2014, ApJ, 793, L3 


\bibitem[Van Eylen et al.(2017)]{vaneylen2017} Van Eylen, V., Agentoft, C., Lundkvist, M.~S., et al.\ 2017, arXiv:1710.05398 

\bibitem[Wu \& Murray(2003)]{Wu2003} Wu, Y., \& Murray, N.\ 2003, \apj, 589, 605 

\bibitem[\protect\citeauthoryear{Wu \& Lithwick}{2011}]{Wu2011} Wu Y., Lithwick Y., 2011, ApJ, 735, 109 

\bibitem[Wu(2018)]{Wu2018} Wu, Y.\ 2018, arXiv:1806.04693 

\end{thebibliography}
